Weyl Law on Asymptotically Euclidean Manifolds

We study the asymptotic behaviour of the eigenvalue counting function for self-adjoint elliptic linear operators defined through classical weighted symbols of order $(1,1)$, on an asymptotically Euclidean manifold. We first prove a two term Weyl formula, improving previously known remainder estimates. Subsequently, we show that under a geometric assumption on the Hamiltonian flow at infinity there is a refined Weyl asymptotics with three terms. The proof of the theorem uses a careful analysis of the flow behaviour in the corner component of the boundary of the double compactification of the cotangent bundle. Finally, we illustrate the results by analysing the operator $Q=(1+|x|^2)(1-\Delta)$ on $\mathbb{R}^d$.

==> biblist.tex <==
\bib{ACS19}{article}{
    author={A. Ascanelli},
    author={S. Coriasco}, 
    author={A. Su\ss}, 
    title={Random-field solutions of linear hyperbolic stochastic partial differential equations with polynomially bounded coefficients}, 
    journal={J. Pseudo-Differ. Oper. Appl.},
    date={2019},
    DOI={10.1007/s11868-019-00290-6},
}

\bib{BaCo11}{article}{
   author={Battisti, U.},
   author={Coriasco, S.},
   title={Wodzicki residue for operators on manifolds with cylindrical ends},
   journal={Ann. Global Anal. Geom.},
   volume={40},
   date={2011},
   number={2},
   pages={223--249},
}

\bib{Cordes}{book}{
	author={Cordes, H.O.},
	title={The technique of pseudodifferential operators},
	date={1995},
	publisher={Cambridge University Press, Cambridge},
}

\bib{CoriascoFIO1}{article}{
   author={Coriasco, S.},
   title={Fourier integral operators in SG classes. I. Composition theorems
   and action on SG Sobolev spaces},
   journal={Rend. Sem. Mat. Univ. Politec. Torino},
   volume={57},
   date={1999},
   number={4},
   pages={249--302 (2002)},
}

\bib{CoriascoFIO2}{article}{
   author={Coriasco, S.},
   title={Fourier integral operators in SG classes. II. Application to SG
   hyperbolic Cauchy problems},
   language={English, with English and Italian summaries},
   journal={Ann. Univ. Ferrara Sez. VII (N.S.)},
   volume={44},
   date={1998},
   pages={81--122 (1999)},
}

\bib{CDS19}{article}{
   author={Coriasco, S.},
   author={Doll, M.},
   author={Schulz, R.},
   title={Lagrangian distributions on asymptotically Euclidean manifolds},
   journal={Ann. Mat. Pura App.},
   pages={DOI 10.1007/s10231-019-00843-y},
   date={2019},
}

\bib{CJT4}{article}{
   author={Coriasco, S.},
   author={Johansson, K.},
   author={Toft, J.},
   title={Global wave-front properties for Fourier integral operators and
   hyperbolic problems},
   journal={J. Fourier Anal. Appl.},
   volume={22},
   date={2016},
   number={2},
   pages={285--333},
}

\bib{CoMa03}{article}{
   author={Coriasco, S.},
   author={Maniccia, L.},
   title={Wave front set at infinity and hyperbolic linear operators with
   multiple characteristics},
   journal={Ann. Global Anal. Geom.},
   volume={24},
   date={2003},
   number={4},
   pages={375--400},
}

\bib{CoMa13}{article}{
   author={Coriasco, S.},
   author={Maniccia, L.},
   title={On the spectral asymptotics of operators on manifolds with ends},
   journal={Abstr. Appl. Anal.},
   date={2013},
   pages={Art. ID 909782, 21 pp},
}

\bib{CoPa02}{article}{
   author={Coriasco, S.},
   author={Panarese, P.},
   title={Fourier integral operators defined by classical symbols with exit
   behaviour},
   journal={Math. Nachr.},
   volume={242},
   date={2002},
   pages={61--78},
}

\bib{CoSc13}{article}{
   author={Coriasco, S.},
   author={Schulz, R.},
   title={The global wave front set of tempered oscillatory integrals with
   inhomogeneous phase functions},
   journal={J. Fourier Anal. Appl.},
   volume={19},
   date={2013},
   number={5},
   pages={1093--1121},
}

\bib{CoSc17}{article}{
   author={Coriasco, S.},
   author={Schulz, R.},
   title={Lagrangian submanifolds at infinity and their parametrization},
   journal={J. Symplectic Geom.},
   volume={15},
   date={2017},
   number={4},
   pages={937--982},
}
	
\bib{DGW18}{article}{
   author={Doll, M.},
   author={Gannot, O.},
   author={Wunsch, J.},
   title={Refined Weyl Law for Homogeneous Perturbations of the Harmonic Oscillator},
   journal={Comm. Math. Phys.},
   volume={362},
   date={2018},
   number={1},
   pages={269--294},
}

\bib{DZ19}{article}{
   author={Doll, M.},
   author={Zelditch, S.},
   title={Schrödinger Trace Invariants for Homogeneous Perturbations of the Harmonic Oscillator},
   journal={J. Spectr. Theory},
   date={to appear},
}

\bib{DuGu75}{article}{
   author={Duistermaat, J. J.},
   author={Guillemin, V. W.},
   title={The spectrum of positive elliptic operators and periodic
   bicharacteristics},
   journal={Invent. Math.},
   volume={29},
   date={1975},
   number={1},
   pages={39--79},
}

\bib{GrRy80}{book}{
   author={Gradshteyn, I. S.},
   author={Ryzhik, I. M.},
   title={Table of integrals, series, and products},
   publisher={Academic Press, New
   York-London-Toronto, Ont.},
   date={1980},
   pages={xv+1160},
   isbn={0-12-294760-6},
}

\bib{GrGr99}{article}{
   author={Grieser, D.},
   author={Gruber, M. J.},
   title={Singular asymptotics lemma and push-forward theorem},
   conference={
      title={Approaches to singular analysis},
      address={Berlin},
      date={1999},
   },
   book={
      series={Oper. Theory Adv. Appl.},
      volume={125},
      publisher={Birkh\"auser, Basel},
   },
   date={2001},
   pages={117--130},
}

\bib{Hormander68}{article}{
   author={H\"ormander, L.},
   title={The spectral function of an elliptic operator},
   journal={Acta Math.},
   volume={121},
   date={1968},
   pages={193--218},
}

\bib{Hormander1}{book}{
   author={H\"ormander, L.},
   title={The analysis of linear partial differential operators. I},
   series={Classics in Mathematics},
   note={Distribution theory and Fourier analysis;
   Reprint of the second (1990) edition [Springer, Berlin;  MR1065993
   (91m:35001a)]},
   publisher={Springer-Verlag, Berlin},
   date={2003},
   pages={x+440},
   isbn={3-540-00662-1},
}

\bib{Hormander3}{book}{
   author={H\"ormander, L.},
   title={The analysis of linear partial differential operators. III},
   series={Classics in Mathematics},
   note={Pseudo-differential operators;
   Reprint of the 1994 edition},
   publisher={Springer, Berlin},
   date={2007},
   pages={viii+525},
   isbn={978-3-540-49937-4},
}

\bib{Hormander4}{book}{
   author={H\"ormander, L.},
   title={The analysis of linear partial differential operators. IV},
   series={Classics in Mathematics},
   note={Fourier integral operators;
   Reprint of the 1994 edition},
   publisher={Springer-Verlag, Berlin},
   date={2009},
   pages={viii+352},
   isbn={978-3-642-00117-8},
}

\bib{MaPa02}{article}{
   author={Maniccia, L.},
   author={Panarese, P.},
   title={Eigenvalue asymptotics for a class of md-elliptic $\psi$do's on
   manifolds with cylindrical exits},
   journal={Ann. Mat. Pura Appl.},
   volume={181},
   date={2002},
   number={3},
   pages={283--308},
}

\bib{MaScSe06}{article}{
   author={Maniccia, L.}, 
   author={Schrohe, E.},
   author={Seiler, J.},
   title={Complex powers of classical SG-pseudodifferential operators},
   journal={Ann. Univ. Ferrara},
   volume={52},
   date={2006},
   pages={353--369},
}

\bib{MaScSe14}{article}{
   author={Maniccia, L.},
   author={Schrohe, E.},
   author={Seiler, J.},
   title={Determinants of classical SG-pseudodifferential operators},
   journal={Math. Nachr.},
   volume={287},
   date={2014},
   number={7},
   pages={782--802},
}

\bib{Melrose92}{article}{
   author={Melrose, R. B.},
   title={Calculus of conormal distributions on manifolds with corners},
   journal={Internat. Math. Res. Notices},
   date={1992},
   number={3},
   pages={51--61},
}

\bib{MelroseGST}{book}{
   author={Melrose, R. B.},
   title={Geometric Scattering Theory, Stanford Lectures},
   publisher={Cambridge University Press, Cambridge, Mass, USA},
   date={1995},
}

\bib{MelroseSST}{article}{
   author={Melrose, R. B.},
   title={Spectral and scattering theory for the Laplacian on asymptotically Euclidian spaces}, 
   conference={
      title={Spectral and scattering theory},
      address={Sanda}, 
      date={1992}
   }, 
   book={
   	series={Lecture Notes in Pure and Appl. Math.}, 
   	volume={161}, 
   	publisher={Dekker, New York}
   }, 
   date={1994}, 
   pages={85--130}
}

\bib{Melrosemwc}{book}{
   author={Melrose, R. B.},
   title={Differential analysis on manifolds with corners},
   note={Unpublished, partly available online at 
   http://www-math.mit.edu/~rbm/book.html, last downloaded 01/08/2016},
}

\bib{MeZw96}{article}{
   author={Melrose, R. B.},
   author={Zworski, M.},
   title={Scattering metrics and geodesic flow at infinity},
   journal={Invent. Math.},
   volume={124},
   date={1996},
   number={1-3},
   pages={389--436},
}

\bib{NiRo}{book}{
   author={Nicola, F.},
   author={Rodino, L.},
   title={Global pseudo-differential calculus on Euclidean spaces},
   series={Pseudo-Differential Operators. Theory and Applications},
   volume={4},
   publisher={Birkh\"{a}user Verlag, Basel},
   date={2010},
   pages={x+306},
   isbn={978-3-7643-8511-8},
}

\bib{SaVa}{book}{
   author={Safarov, Yu.},
   author={Vassiliev, D.},
   title={The asymptotic distribution of eigenvalues of partial differential
   operators},
   series={Translations of Mathematical Monographs},
   volume={155},
   note={Translated from the Russian manuscript by the authors},
   publisher={American Mathematical Society, Providence, RI},
   date={1997},
   pages={xiv+354},
   isbn={0-8218-4577-2},
}

\bib{Schrohe88}{article}{
   author={Schrohe, E.},
   title={Complex powers on noncompact manifolds and manifolds with
   singularities},
   journal={Math. Ann.},
   volume={281},
   date={1988},
   number={3},
   pages={393--409},
}

\bib{Wunsch99}{article}{
   author={Wunsch, J.},
   title={The trace of the generalized harmonic oscillator},
   language={English, with English and French summaries},
   journal={Ann. Inst. Fourier (Grenoble)},
   volume={49},
   date={1999},
   number={1},
   pages={viii, xi--xii, 351--373},
}


